A cryogenic continuously rotating half-wave plate for the POLARBEAR-2b cosmic microwave background receiver

We present the design and laboratory evaluation of a cryogenic continuously rotating half-wave plate (CHWP) for the POLARBEAR-2b (PB-2b) cosmic microwave background (CMB) receiver, the second installment of the Simons Array. PB-2b will observe at 5,200 m elevation in the Atacama Desert of Chile in two frequency bands centered at 90 and 150 GHz. In order to suppress atmospheric 1/f noise and mitigate systematic effects that arise when differencing orthogonal detectors, PB-2b modulates linear sky polarization using a CHWP rotating at 2 Hz. The CHWP has a 440 mm clear aperture diameter and is cooled to $\approx$ 50 K in the PB-2b receiver cryostat. It consists of a low-friction superconducting magnetic bearing (SMB) and a low-torque synchronous electromagnetic motor, which together dissipate < 2 W. During cooldown, a grip-and-release mechanism centers the rotor to < 0.5 mm, and during continuous rotation, an incremental optical encoder measures the rotor angle with a noise level of 0.1 $\mathrm{\mu rad / \sqrt{Hz}}$. We discuss the experimental requirements for the PB-2b CHWP, the designs of its various subsystems, and the results of its evaluation in the laboratory. The presented CHWP has been deployed to Chile and is expected to see first light on PB-2b in 2020 or 2021.

==> scratch.tex <==
INTRO

remain one the most powerful and versatile observational tools of modern cosmology. While CMB temperature anisotropies are the bedrock of the standard cosmological model \cite{bennett_four-year_1996,hinshaw_nine-year_2013,planck_collaboration_planck_2019}, CMB polarization has

While temperature fluctuations shaped much of our current understanding of modern cosmology and are used to study secondary distortions,  \cite{sunyaev_observations_1972,lewis_weak_2006}, polarization fluctuations are the predominant channel to study both the early universe and it's history

While CMB temperature anisotropies are the bedrock of the standard cosmological model \cite{bennett_four-year_1996,hinshaw_nine-year_2013,planck_collaboration_planck_2019}

On degree scales, B-modes are thought to be generated by a stochastic background of primordial gravitational waves sourced by inflation, a theorized period of rapid space-time expansion $\sim 10^{-30}$ after the Big Bang~\cite{guth_inflationary_1981,seljak_direct_1999,zaldarriaga_all-sky_1997}.

Even though the stator load exceeded the expectation during lab testing, the rotor temperature and resulting 4~K load were within specifications, validating two key aspects of the thermal model. Additionally, the CHWP continuous rotation had no affect on the PTR second cooling stage or 4~K shell temperatures, demonstrating that the PB-2b optics tube is robust to excess CHWP loads.

The CHWP retrofits into the heritage PB-2b design without disturbing other experiment subsystems. 

The stator is an assembly of the motor, encoder, YBCO stator, and other auxiliary parts on the stator baseplate. The stator baseplate is bolted to the 50~K shell via 58 1/4-20 fasteners, which is in turn connected via a custom heatstrap to the optics tube's first PTC stage. The CHWP system is designed to direct power dissipation to the stator in order to minimize rotor heating. However, if we dump too much power onto the stator, it will warm the 50~K assembly, which in turn loads the 4~K stage. As discussed in Section \ref{sec:requirements}, we require that the waveplate increase the first-stage PTC temperature by < 1 K, which according to measured PTC load curves means that the HWP system must dissipate < 2 W. 

Stator power sources include encoder LED dissipation, motor solenoid dissipation, and rotor friction. The encoder has a total of ten LEDs, as described above, and each LED dissipates $\approx$ 80 mW of power during normal operation; therefore 800 mW of power is dissipated by the LEDs alone, which is the largest source of loading on the stator. The motor consists of 114 coils, and each dissipates $\approx$ 1.6 mW, totaling 180 mW of motor power. Lastly, the rotor, which is spinning at 2 Hz, has azimuthal variation in its magnetic field--both due to rotor magnet imperfections and due to the magnetic sprockets--and these variations lead to both Eddy dissipation in the stator and hysteresis loss in the YBCO. At 2 Hz, this dissipation is measured to be 80 mW via spin-down testing with the motor powered off, as described in Section \ref{sec:bearing_thermal_performance}. Both the motor power dissipation and rotor friction vs frequency, as measured in the lab, is shown in Figure \ref{fig:rot_pow_diss}. 

Variation in rotor temperature leads to variation in the detector optical power due to variable thermal emission from the sapphire and its AR coating. Because this variation is not modulated by the CHWP, it is ideally rejected by the demodulation routine. However, the detectors are not perfectly linear and their CHWP-synchronous gain is not perfectly reconstructed, and therefore 0$f_{\mathrm{HWP}}$ optical fluctuations can couple to that of 4$f_{\mathrm{HWP}}$, injecting additional 1/f noise into the demodulated data~\cite{takakura_performance_2017}. Some of the 0$f_{\mathrm{HWP}}$ projection onto 4$f_{\mathrm{HWP}}$ can be removed using principle component analyses, but in order to achieve 1/f knees down to $\sim$~10~mHz, thermal fluctuations in the optical system, including that of the CHWP, must be carefully controlled. We leverage measurements made by POLARBEAR~\cite{takakura_performance_2017} to estimate emission from the primary mirror and the detector non-linearity it induces, and we simultaneously impose requirements on the thermal stability of all optical elements and on the stability of the detector electrical bias. We set an RMS rotor temperature stability requirement of of 0.5~K at 50~mHz, or over 20~s timescales.

\begin{equation}
    \frac{\mathrm{d} P_{\mahrm{opt}}}{\mathrm{d} T_{\mathrm{CMB}}} = \eta_{\mathrm{tel}} \int_{\nu_{1}}^{\nu_{2}} \left[ \frac{1}{k_{\mathrm{B}}} \left(  \frac{h \nu}{T_{\mathrm{CMB}} \left( \exp \left[ h \nu / k_{\mathrm{B}} T_{\mathrm{CMB}} \right] - 1 \right) } \right)^{2} \exp \left[h \nu / k_{\mathrm{B}} T_{\mathrm{CMB}} \right] \right] \mathrm{d} \nu \; ,
    \label{eq:cmb_conv}
\end{equation}

Thermal emission from the CHWP sapphire is simulated~\cite{hill_bolocalc_2018} to load the detectors with $8 \times 10^{-16}$~W of power at 150~GHz~\footnote{The CHWP thermal emission in the 90~GHz band is smaller, and therefore we focus on the 150~GHz band to set the most stringent requirement.}. Power variation due to CHWP temperature variation can be written as
\begin{equation}
    \frac{\mathrm{d} P_{\mathrm{opt}}}{\mathrm{d} T_{\mathrm{HWP}}} = \int_{0}^{\infty} \epsilon_{\mathrm{HWP}}(\nu) \frac{\mathrm{d} B(\nu, T)}{\mathrm{d} T} \bigg\rvert_{T_{\mathrm{HWP}}} \eta_{\mathrm{rcvr}}(\nu) \mathrm{d} \nu \; ,
    \label{eq:chwp_power}
\end{equation}
\noindent
where $P_{\mathrm{opt}}$ is the optical power on a 150~GHz detector, $\epsilon_{\mathrm{HWP}}(\nu)$ is the HWP emissivity, $B(\nu, T)$ is the Planck power spectrum, $\eta_{\mathrm{rcvr}}(\nu)$ is the receiver's optical efficiency between the CHWP and the detector, and $T_{\mathrm{HWP}} = 50$~K. This coefficient is simulated to be $\mathrm{d} P_{\mathrm{opt}} / \mathrm{d} T_{\mathrm{HWP}} = 2 \times 10^{-17}$~W/K.

In turn, this CHWP temperature fluctuation can be converted to an equivalent CMB temperature fluctuation as
\begin{equation}
    \frac{\mathrm{d} T_{\mathrm{CMB}}}{\mathrm{d} P_{\mathrm{opt}}} = \left[ \int_{0}^{\infty} \frac{\mathrm{d} B(\nu, T)}{\mathrm{d} T} \bigg\rvert_{T_{\mathrm{CMB}}} \eta_{\mathrm{tel}}(\nu) \mathrm{d} \nu \right]^{-1}
    \label{eq:tcmb_popt}
\end{equation}
\noindent
where $\eta_{\mathrm{tel}}$ is the optical efficiency of the full telescope and receiver system, and $T_{\mathrm{CMB}} = 2.7$~K. This factor is calculated to be $\mathrm{d} T_{\mathrm{CMB}} / \mathrm{d} P_{\mathrm{opt}} = 1.2 \times 10^{13}$~$\mathrm{K_{CMB}}$/W.

Microphonics are especially pronounced at low frequencies, and while the focal plane structure is stiff and measured to have a high-pass cutoff frequency of $\approx$~80~Hz,, and it is desirable that any CHWP mechanical resonances be high in frequency and low in amplitude. 

The IRIG signal is GPS synchronized to < 40~ns and is sampled once per second, and its jitter RMS is consistent with the Arduino noise floor. The encoder jitter is $\approx$~90~$\mathrm{\mu s}$ (or 0.02 \%) $f_{\mathrm{HWP}}$, and shows other rotation-synchronous structures. Both signals are drifting slightly over this timescale, which is also due to the 1/f noise of the Arduino timers. 

``Jitter'' is defined to be clock/angle vs time after a second-order polynomial subtraction, except for the angle template subtraction, which also subtracts a revolution-synchronous jitter template. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\linewidth, trim=0cm 1.3cm 0cm 2cm, clip]{Figures/encoderJitter_tod.pdf}
    \caption{A three second sample of polynomial-subtracted jitter for the IRIG clock and angle encoder clock. The HWP is rotating at $\approx$ 2.2~Hz and is sampled 1,140 times per rotation. The IRIG signal is GPS synchronized to < 40~ns and is sampled once per second, and its jitter RMS is consistent with the Arduino noise floor. The encoder jitter is $\approx$~90~$\mathrm{\mu s}$ (or 0.02 \%) $f_{\mathrm{HWP}}$, and shows other rotation-synchronous structures. Both signals are drifting slightly over this timescale, which is also due to the 1/f noise of the Arduino timers.}
    \label{fig:jitter_tod}
\end{figure}

In addition to lensing B-modes, galactic synchrotron radiation and thermal dust emission create their own B-mode foreground. 

It is designed to measure arcminute scales over large sky areas, enabling simultaneous characterization of primordial and lensing B-modes. It also covers a wide frequency range, allowing CMB and galactic polarization components to be separated. 

~\footnote{In theory, the modulated signal due to CHWP temperature variations could be measured and subtracted. However, such a delineation would require exquisitely precise HWP temperature monitoring, which is challenging to implement for a rotating optic.}

\footnote{We expect the PB-2b CHWP thermal signal to be smaller than that of the POLARBEAR HWP for two configurational reasons. First, sapphire emission is a steep function of temperature, and therefore, the fractional 4$f_{\mathrm{HWP}}$ signal due to differential thermal emission between the two sapphire crystal axes at non-normal incidence will be smaller at cryogenic temperatures. Second, the POLARBEAR HWP is located near the primary focus where each detector pixel illuminates a small region on its surface. This configuration amplifies HWP-synchronous signals due to localized optical non-idealities to a greater extent than that of the PB-2b CHWP.}

outer diameter is 528 mm, its

, its height is 19 mm, 

can be modeled using paramagnetic forces and follows a 

power-law dependence on 

However, the SMB is only engaged below the YBCO's superconducting transition temperature. Therefore, the rotor must be suspended above the stator when warm and released for rotation when cold.

1120~turns, 

that poke through the slotted encoder plate

The board's overall size is 300~mm x 230~mm.

digital using a comparator, whose threshold is tuned via a potentiometer. The digital 

The driver board converts the angle encoder digital waveform to a DC voltage using frequency-to-voltage converter whose output is sent to the PID, which in turn controls the H Driver DC power supply.

Efficiency loss due to increasing rotation frequency arises from an inductive phase shift between the solenoid voltage bias and the solenoid current, causing the stator's rotating magnetic field to lag behind that of the rotor.

Efficiency loss due to misalignment arises from increased distance between the stator's solenoids and rotor's magnet sprockets, weakening the motor coupling. 

Another core principle of the CHWP system is precise reconstruction of the rotor angle. In PB-2b, the CHWP is located behind both of the telescope's off-axis, ambient-temperature mirrors, which introduce instrumental polarization that is modulated by the CHWP. This spurious HWP-synchronous signal, if stable, can be removed during demodulation if the CHWP angle is known precisely. However, imperfect angle measurement leads to imperfect demodulation, which injects white and/or 1/f noise into the demodulated detector data~\cite{takakura_performance_2017}. Therefore it is critical to measure the CHWP angle precisely enough to make this angle-jitter noise subdominant to that of other detector noise sources, such as photon noise. As discussed, in Section \ref{sec:requirements}, the angle noise requirement is < 1 $\mathrm{\mu s \ \sqrt{Hz}}$, which drives the angle encoder design.

The primary challenge for the CHWP angle encoder readout is managing noise, glitches, and latency in the cabling and driver board electronics. We use double-shielded Alpha Wire \footnote{http://www.alphawire.com/} to carry the photocurrent signals from the receiver cryostat to the driver PCB, and the driver board uses carefully chosen low-pass-filtered feedback for the photocurrent transimpedance amplifiers as well as an analog-digital-separated ground-plane scheme to keep the encoder signals free of high-frequency artifacts.

mapping speed does not depend steeply on rotor temperature near 50~K. However, the radiative load on the 4~K stage is dictated by the rotor temperature, and an increase in the temperature of downstream optical elements, such as the lenses and the Lyot stop, can have dramatic impacts on experimental sensitivity. T

While we did not see substantial CHWP rotor warm-up during PB-2b lab evaluation (see Section \ref{sec:thermal_performance}), if such warming is suspected, the temperature can be checked between observation cycles. The motor is capable of spinning the rotor down in $\approx$~5~min and up in $\approx$~30~min. The detector array's millikelvin fridge must be cycled for a few hours each day, offering a window to halt rotation, touch the flex circuit with the gripper to read the diode thermometer, and release with plenty of time to restart before observations resume. This procedure is not part of normal operations but offers some insurance against unexpected thermal behavior in the field.

The angle encoder signal is amplified and digitized on the motor driver board before being acquired by the MCU, which also acquires an IRIG-B input and sends packets of each data stream to an external computer.

it effectively measures the Arduino's 1/f noise below 0.5~Hz. The IRIG and encoder jitters' low-frequency 

are nearly identical and semi-correlated down to $10^{-2}$~Hz,

, despite the Arduino drifts

Magnetic pickup at 4$f_{\mathrm{HWP}}$ mimics modulated sky polarization

The simulated rotor-generated RMS magnetic field at the focal plane, which is 1.8~m from the CHWP, is 500~$\mathrm{\mu}$G, orders of magnitude below the variation expected from rotating the telescope through the Earth's magnetic field. Even so, rotation synchronous signals can contaminate the demodulated detector data, and therefore we characterize the CHWP-induced magnetic field and discuss the results here.

at a $\sim$~10~$\mathrm{\mu G}$ noise level

Additionally, no CHWP-induced amplifier noise or artifacts were observed in the time streams. 

This result suggests that the PB-2b detectors may be less sensitive to ambient fields than assumed in Sec.~\ref{sec:noise_requirements}, which in turn suggests that the 4$f_{\mathrm{HWP}}$ magnetic interference may be further beneath the detector-array noise floor than the LBNL measurement indicates.

and warmed the 50~K stage by 1.3~K, which is larger than the 1~K allocation. 

given the improved heat sinking technique, 

The PB-2a data is used to represent expected IR absorbing filter temperature variations in the field---which are substantially larger than those measured in the lab---and include changes in telescope elevation, which affect PTR efficiency. 

In the remote event of a UPS failure, the rotor stops on its own and settles onto PTFE crash pads on the retaining ring (see Fig.~\ref{fig:chwp_tabletop}). To re-center the rotor after power restoration, the receiver is positioned horizontally, and the bottom gripper finger---which has a slight ``v'' shape about the radial direction to keep the rotor from rolling side-to-side---centers the rotor before the top two motors engage. This procedure was tested at LBNL and re-centered the rotor to <~1~mm. We also tested this procedure with the PB-2b receiver warm and open at UCSD to confirm both the behavior of the automated control software and the quality of the gripper finger-to-rotor groove interface after recovery.

The thermal circuit consists of the IR filter, rotor, encoder, and motor, which are at 50 K, and the field lens, which is at 4 K. 

Because the IRF absorbs radiation from 300~K, maximizing the IRF conductivity to the stator $k_{2}$ is key to controlling the rotor temperature. The alumina filter is heat strapped to its fixture plate using 24 ribbons of 99.9999\% purity aluminum, which has superior conductivity between 100$\sim$50 K, is malleable enough to engage the alumina surface without thermal grease, and is flexible enough to absorb differential thermal contraction between the alumina filter and the aluminum fixture. The fixture plate is machined from aluminum 1100 and is bolted to six titanium-helicoiled OFHC copper towers, which provide a thermal path to the stator baseplate. The measured conductivity between the absorbing filter and the stator baseplate of $k_{2} = 2.5$~W/K is enough to keep the filter < 10 K warmer than the 50 K stage.

Because the IRF absorbs radiation from 300~K, maximizing the IRF conductivity to the stator $k_{2}$ is key to controlling the rotor temperature.

n $2 \; \mathrm{Hz} \times 38 \; \mathrm{slots} =$ 

Using the values in Table \ref{tab:thermal_values}, we run three analytic simulations: (1) the total load on the rotor vs rotor temperature, (2) the total load on the stator vs rotor temperature, and the (3) the CHWP-induced load on the field lens vs the total load on the rotor. The results of (1) and (3) are shown in Figure \ref{fig:rotor_temp}. The zero-crossings for the rotor load correspond to the model expectations, with the solid line denoting the median and the shaded regions denoting the 95\% confidence interval. Loading excesses on the rotor can come from light leaks into the CHWP assembly most notably through the gripper ports, and loading deficits on the rotor can come from most notably from inaccurate model assumptions, such as the transmissivity of the vacuum window, RT-MLI, or the alumina IR filter.

Galactic synchrotron radiation produces B-modes with a falling mm-wave spectrum,\cite{} while thermal emission from interstellar dust produces B-modes with a rising spectrum.\cite{}

While lensing B-modes are detected with high significance,\cite{wu_measurement_2019,the_polarbear_collaboration_measurement_2017,keisler_measurements_2015,the_planck_collaboration_planck_2016}

Delensing has been demonstrated using external data sets to trace gravitational structure,\cite{} but CMB lensing measurements must continue to improve as the bound on primordial B-modes tightens.

its polarized input amplitude modulates the HWP-generated carrier, and if rotated rapidly enough, 

This sensitivity degradation is suppressed by cooling the HWP to low temperatures, and t

 Its requirements are divided into spatial/optical, thermal, noise, and operational categories.
 
 The rotor temperature determines both the optical stack's mm-wave emission onto the detectors and its infrared (IR) emission onto the field lens.
 
 Additionally, POLARBEAR and the Atacama B-mode Search (ABS) operate in Chile and measure an intensity 1/f knee of 1$\sim$2~Hz at 150~GHz.
 
 Note that this requirement is five orders of magnitude below the Earth's 3~G  peak-to-peak magnetic field at the Chilean site.\footnote{https://www.ngdc.noaa.gov/geomag/calculators/magcalc.shtml\#igrfwmm}
 
 even in the absence of top two grippers.
 
 While all three gripper subassemblies are used in parallel during normal CHWP operation, the ability of the bottom gripper finger to align the rotor on its own
 
 the second installment of the Simons Array
 
 of E-modes
 
 , which does not out-motivate the 50~K benefits discussed in Sec.~\ref{sec:chwp_design}.
 
 ---such as rotor angle measurement error and HWP-synchronous magnetic and thermal signals---
 
 38 TESs are digital-frequency-domain multiplexed\cite{dobbs_frequency_2012} on each SQUID between 1 and 5~MHz.
 
 Rotor temperature monitoring is particularly important and is discussed in Sec.~\ref{sec:rotor_thermometry}
 
 A detailed discussion of the CHWP optical stack's design, evaluation, and systematic effects will be presented in future publications.
 
 focuses on system operation---including gripper interfacing, cryo-mechanical robustness, rotational stability, magnetic interference, and control software validation---
 
 As described in Sec.~\ref{sec:requirements}, encoder noise must be $< \; 7 \; \mathrm{\mu rad / \sqrt{Hz}}$ to cleanly demodulate the detector data.
 
 In the following subsections, we discuss the performance of various CHWP subsystems during different operational modes, including cooldown, spin-up, continuous rotation, and shutdown/recovery.
 
 The CHWP thermal performance is evaluated in two stages. First, we measure rotor friction and solenoid dissipation in the LBNL dark cryostat. The rotor's friction is evaluated by measuring frequency vs time as it spins down with the motor turned off. The motor's dissipation is evaluated by measuring the current through and resistance of the solenoids. The rotor and motor heating as a function of frequency are shown in Fig.~\ref{fig:rot_pow_diss}, and at a 2~Hz, rotor dissipation is 80~mW and motor dissipation is <~200~mW. A fit to the rotor friction curve shows that most loss is due to eddy currents. The motor dissipation's steep slope is due to decreasing motor efficiency and increasing rotor frictional at higher frequencies. The error bars on the motor dissipation are fractional and quantify motor efficiency uncertainty due to rotor-stator alignment and stator temperature, which determines solenoid resistance.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\linewidth, trim=0.5cm 1cm 2cm 2.5cm, clip]{Figures/rotor_motor_dissipation.pdf}
    \caption{Measured rotation-frequency-dependent dissipation during CHWP continuous rotation. Rotor friction is predominantly due to eddy losses, and motor dissipation is due to resistive heating in the solenoid array. The motor-dissipation error bars represent possible variations due to rotor positioning, solenoid temperature, and cryostat angle.}
    \label{fig:rot_pow_diss}
\end{figure}

Second, we evaluate cryo-optical performance in a test configuration of the PB-2b receiver at UCSD, as shown in Fig.~\ref{fig:chwp_in_pb2b}. Even though in this configuration the IRF, HWP, and lenses are without AR coatings, bare alumina and sapphire are still largely IR black, and therefore this PB-2b test configuration can be used to evaluate the accuracy of the CHWP thermal model presented in Sec.~\ref{sec:thermal_design} and App.~\ref{app:thermal_sim}. 

During UCSD testing, the CHWP rotor thermometer disconnected, leaving us to instead infer the rotor temperature rather than monitor it directly. Using a load curve of the field lens\cite{howe_polarbear-2_2019} and comparing field lens and 50~K temperatures to a dark run without the CHWP,\cite{howe_polarbear-2_2019} we measure a rotor temperature of <~50~K and a field lens temperature of 6.4~K, both of which are slightly better than the thermal model's prediction in the presence of no AR coatings. However, the measured 50~K load is $\approx$~2.5~W, which is larger than the 2~W requirement and 1.3~W expectation. This test was performed before adopting the solenoid heat sinking scheme described in Sec.~\ref{sec:thermal_design}, which has shown to reduce solenoid temperatures by > 5x in auxiliary tests. Therefore, we anticipate a < 2~W stator load when the CHWP is deployed to Chile.

Finally, we evaluate any CHWP-induced heating of the focal plane. The focal plane structure is an $\sim$~80~Hz high-pass filter,\cite{howe_polarbear-2_2019} and the CHWP rotor has a resonant frequency of $\sim$~130~Hz, both of which are much higher than the 2~Hz rotation frequency. We turn the CHWP on and off at various drive voltages over the course of several hours, and we see no focal plane temperature changes to within the $\sim$~0.3~mK/hr background drift of the mK thermometry.\footnote{Note that no focal plane temperature regulation was employed during this test, and therefore this background drift is larger than that which is achievable.}

To evaluate thermal stability, we simulate rotor temperature using the thermal model presented in Sec.~\ref{sec:thermal_design} and App.~\ref{app:thermal_sim}. The rotor's temperature variations are dominated by those of the 50~K stage to which it is radiatively tied. These variations are expected to be very slow, because the rotor has a $\approx$~900~J/K heat capacity and a $\approx$~10~mW/K coupling to its surroundings at 50~K. Due to diurnal ambient variations and changes in telescope elevation---which impact PTR performance---50~K temperature drifts in Chile are substantially larger than in the lab. Therefore, we use 24 hours of 50~K temperature data from the field\footnote{We obtain field data from PB-2a, which is currently observing in Chile} to simulate the expected rotor stability. The measured 50~K-stage and simulated rotor power spectra are shown in Fig.~\ref{fig:hwp_stability}. The rotor acts as a low-pass filter, and its simulated drift is $\approx$~0.3~$\mathrm{mK / \sqrt{Hz}}$ at 1~mHz, which is below the 1~$\mathrm{mK / \sqrt{Hz}}$ requirement. We note that rotor temperature stability can be improved substantially by regulating the 50~K stage temperature, which may be desirable for future experiments with tighter noise requirements.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\linewidth, trim=0.3cm 1cm 2.4cm 2.5cm, clip]{Figures/rotor_tempVariation_pb2a_psd.pdf}
    \caption{Power spectrum of measured 50~K temperature variations in Chile, along with that of simulated rotor temperature variations. The rotor's large thermal mass and small radiative coupling make it an effective low-pass filter, suppressing IR filter fluctuations by >~100x at 1~mHz.}
    \label{fig:hwp_stability}
\end{figure}

These requirements ensure effective 1/f noise mitigation while not degrading key PB-2b performance metrics, such as those of the optics, cryogenics, and detectors.

 The vacuum window is not shown but is located just beyond the image's top edge.
 
 The optics tube's 50~K heat strap has a conductivity of $\approx$~2~W/K,
 
 To estimate the expected PB-2b I-to-P amplitude, we note that
 
 and the rotor's 5~mm clearance (see Sec.~\ref{sec:motor_eff})
 
 Even though this buckling reduces the YBCO thermal contact, we measure a <~3~K differential between it and the stator baseplate.
 
 The encoder LEDs are hidden beneath the slotted encoder plate, but an unfastened photodiode read head is resting above it at the photo's bottom right.
 
 Finally, each motor's pushing force is empirically tuned to hold the rotor firmly enough for adequate thermal contact while not unnecessarily stressing the gripper arms.
 
 its radiative coupling to 4~K lowers its temperature below that of the IRF, just like with
 
 When stationary, the CHWP should also introduce minimal power onto the 50~K stage, with the primary load increase coming from gripper-port light leaks (see Sec.~\ref{sec:gripper_design}), which are together estimated to be <~10~mW.
 
 To minimize ring-magnet hysteresis losses, we only use non-magnetic\footnote{Stainless steel (SS) is weakly magnetic, and therefore we avoid using SS hardware near the ring magnet as well.} hardware within 20~mm of the rotor, employing brass and titanium fasteners where appropriate. To align the rotor's inertial and rotational axes, we use dowel pins to assemble the ring magnet, rotor stage, slotted encoder plate, sprocket ring, and optical stack, as even a $\approx$~10~g inertial imbalance significantly degrades motor performance.
 
 The following subsections discuss, start-up, continuous rotation, thermal performance, and shutdown and recovery.
 
 and the encoder's white-noise noise level (see Sec.~\ref{sec:encoder_jitter})
 
 In the presented data, the encoder's white noise is limited by the Arduino clock rate, and its low frequency noise is limited by Arduino stability. Additionally, Arduinos are not always reliable and are particularly vulnerable to the extreme conditions of the Chilean observation site. In an effort to improve system robustness, we replace the Arduino with a BBB MCU, which has a 200~MHz clock that is shared by two PRUs, as described in Sec.~\ref{sec:angle_encoder}.
 
 In addition, the BBB clock is ten times faster, enabling better timing resolution, and is electrically and mechanically robust, which are important qualities for site operations.
 
 Because the IRIG signal is very stable, $\delta \tau_{\mathrm{clk}}^{\mathrm{IRIG}}$ measures the Arduino's 1/f noise.  The 0.03\%/hr rotational stability (see Fig.~\ref{fig:rot_stability}) results in sharp $f_{\mathrm{HWP}}$ peaks with no visible side bands. 
 
 1.5~m away from the CHWP, which is 
 
 While $1 f_{\mathrm{HWP}}$ and $2 f_{\mathrm{HWP}}$ variations are clear,
 
 focal plane structure is an $\sim$~80~Hz high-pass filter\cite{howe_polarbear-2_2019} and
 
 $\delta \tau_{\mathrm{clk}}$ as the IRIG MCU clock value $\tau_{\mathrm{clk}}^{\mathrm{IRIG}}$ vs. IRIG time $t$ minus a quadratic fit $P_{\mathrm{fit}}^{\tau}$
 
 The top panel of Fig.~\ref{fig:jitter_psd} shows power spectral densities (PSDs) for the IRIG and encoder clock jitters. 
 
 The effectiveness of the template in Eq.~\ref{eq:template} applied across $N_{\mathrm{rev}} \approx$~8,000 is a promising indication that both optical and pathological HWP-synchronous signals in the field can be precisely characterized and  
 
  A unique property of the SMB is that it does not wobble, even if it is gravitationally imbalanced. Therefore the observed $f_{\mathrm{HWP}}$ angle jitter is caused by the slotted encoder plate and magnet ring being slightly non-concentric, while higher-frequency jitter structures are caused by non-uniform patterning of the encoder slots.
  
   in Fig.~\ref{fig:jitter_psd}, the 1/f noise in the angle and IRIG jitter spectra are highly correlated, suggesting that their origins are on the MCU rather than within the CHWP encoder electronics
   
   This change in spectral shape also appears in the broadening of the $1 f_{\mathrm{HWP}}$ peak

noise in $\tau_{\mathrm{Enc}}$ and $\tau_{\mathrm{IRIG}}$ and therefore propagates to the angle jitter. 

measures the 1/f noise of its MCU clock and

, better revealing the noise floor

1/f noise is dominated by Arduino clock drift, and the angle jitter white noise floor is $\sim$~0.1~$\mathrm{\mu rad / \sqrt{Hz}}$. The sharpness of the $f_{\mathrm{HWP}}$ peaks exhibit excellent rotation stability, and the forest of harmonics is largely subtracted by a simple revolution-synchronous template.

the $2 \pi$-repeating encoder template

shows a similar slope to that of $\delta \chi_{\mathrm{HWP}}^{\mathrm{poly}}$ >~0.1~Hz, while <~0.1~Hz the $\delta \chi_{\mathrm{HWP}}^{\mathrm{poly}}$ spectrum steepens due to drifts in $f_{\mathrm{HWP}}$. Even in the frequency region where their slopes are similar, the IRIG and angle jitter spectra are uncorrelated, revealing that $\tau_{\mathrm{Enc}}$ and $\tau_{\mathrm{IRIG}}$ are drifting independently.

This noise level is consistent with the Arduino's timing resolution, and therefore we expect even better white-noise performance with the BBB, whose clock is >~10x faster.

while the $2 \pi f_{\mathrm{HWP}} \delta \tau_{\mathrm{IRIG}}^{\mathrm{poly}}$ spectrum shows the Arduino's 1/f noise below 0.5~Hz.the $2 \pi f_{\mathrm{HWP}} \delta \tau_{\mathrm{IRIG}}^{\mathrm{poly}}$ spectrum shows the MCU noise properties and how those propagate to the angle measurement

jitter $\delta \chi^{\mathrm{poly}}_{\mathrm{HWP}}$ and $\delta \chi^{\mathrm{temp}}_{\mathrm{HWP}}$ as well as of the IRIG clock jitter $\delta \tau_{\mathrm{IRIG}}^{\mathrm{poly}}$

are well characterized by $A(\chi)$

Additionally, these rotation-synchronous structures are measured with high signal-to-noise, allowing them to be effectively subtracted during detector demodulation and data analysis. Because

The figure's inset zooms in on the $1 f_{\mathrm{HWP}}$ peak, better displaying its shape and side-band power.

suggesting that the 1/f noise in this region is dominated MCU clock drifts

as best shown in the $1 f_{\mathrm{HWP}}$ inset,

Below $\sim$~0.02~Hz, drifts in $f_{\mathrm{HWP}}$ begins to dominate, injecting excess angle jitter power into the $\delta \chi_{\mathrm{HWP}}$ spectra.

\iffalse
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.98\linewidth, trim=0.5cm 1.3cm 0.3cm 3.3cm, clip]{Figures/encoderJitter_tod.pdf}
    \caption{A three-second sample of clock jitter for the IRIG and angle encoder signals. The rotor is spinning at $\approx$~2.2~Hz and is sampled 1,140 times per revolution.}
    \label{fig:jitter_tod}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.98\linewidth, trim=9.9cm 4.2cm 10.2cm 4cm, clip]{Figures/encoderJitter_psd.pdf}
    \caption{Power spectral densities (PSDs) of the IRIG and encoder MCU clock jitter (top) and of the angle jitter (bottom) during one hour of continuous rotation in the LBNL cryostat. 1/f noise is dominated by Arduino clock drift, and the angle jitter white noise floor is $\sim$~0.1~$\mathrm{\mu rad / \sqrt{Hz}}$. The sharpness of the $f_{\mathrm{HWP}}$ peaks exhibit excellent rotation stability, and the forest of harmonics is largely subtracted by a simple revolution-synchronous template.}
    \label{fig:jitter_psd}
\end{figure}
\fi

The CHWP is assumed to have an epoxy-based AR coating,\cite{rosen_epoxy-based_2013} while the WHWP is assumed to have a plastic AR coating. The mapping speed decrease with increasing HWP temperature is primarily due to increasing mm-wave emission, which in turn increases detected photon noise. Some of the sensitivity loss at ambient temperature can be reclaimed by using a more transparent AR coating, such as that of the PB-2a WHWP, but the biggest sensitivity gain comes from cooling the HWP to cryogenic temperatures.

wired via a custom 10~mm x 10~mm printed wiring board

It uses a CHWP to suppress 1/f contamination due to atmospheric turbulence and
to allow a single polarimeter to measure both polarization states, mitigating systematic effects that arise when differencing orthogonal detectors.

, rejecting unpolarized atmospheric fluctuations and allowing a single polarimeter to measure both polarization states

The rotor fits around this aperture tube and has an inner diameter of 470~mm.

Additionally, modeling uncertainties without AR coatings are larger than with them, as PB-2b's coating materials are IR black.\cite{inoue_cryogenic_2014, halpern_far_1986}

. Because 1$f_{\mathrm{HWP}}$ signals are undetected in the dark bolometers, 

. The motor is low-torque and azimuthally symmetric, the bearing is highly uniform and low-friction, and the rotor has a large moment of inertia. Therefore, rotation is stable over hundreds of revolutions, 
